Latent Diffusion, Implicit Amplification: Efficient Continuous-Scale Super-Resolution for Remote Sensing Images

Recent advancements in diffusion models have significantly improved performance in super-resolution (SR) tasks. However, previous research often overlooks the fundamental differences between SR and general image generation. General image generation involves creating images from scratch, while SR focuses specifically on enhancing existing low-resolution (LR) images by adding typically missing high-frequency details. This oversight not only increases the training difficulty but also limits their inference efficiency. Furthermore, previous diffusion-based SR methods are typically trained and inferred at fixed integer scale factors, lacking flexibility to meet the needs of up-sampling with non-integer scale factors. To address these issues, this paper proposes an efficient and elastic diffusion-based SR model (E$^2$DiffSR), specially designed for continuous-scale SR in remote sensing imagery. E$^2$DiffSR employs a two-stage latent diffusion paradigm. During the first stage, an autoencoder is trained to capture the differential priors between high-resolution (HR) and LR images. The encoder intentionally ignores the existing LR content to alleviate the encoding burden, while the decoder introduces an SR branch equipped with a continuous scale upsampling module to accomplish the reconstruction under the guidance of the differential prior. In the second stage, a conditional diffusion model is learned within the latent space to predict the true differential prior encoding. Experimental results demonstrate that E$^2$DiffSR achieves superior objective metrics and visual quality compared to the state-of-the-art SR methods. Additionally, it reduces the inference time of diffusion-based SR methods to a level comparable to that of non-diffusion methods.

==> tables/real-world.tex <==
\begin{table}[htbp]
    \centering
    \caption{Add caption}
    \begin{tabular}{cccc}
        \toprule
        \toprule
        Category                                                 & Methods & NIQE & BRISQUE \\
        \midrule
        Baseline                                                 & Bicubic &      & \\
        \midrule
        \multicolumn{1}{c}{\multirow{3}[2]{*}{Regression-based}} & LIIF    &      & \\
        & SADN    &      & \\
        & HAT-L   &      & \\
        \midrule
        \multirow{2}[2]{*}{GAN-based}                            & ESRGAN  &      & \\
        & SPSR    &      & \\
        \midrule
        \multicolumn{1}{c}{\multirow{4}[2]{*}{Diffusion-based}}  & SR3     &      & \\
        & EDiffSR &      & \\
        & IDM     &      & \\
        & Ours    &      & \\
        \bottomrule
        \bottomrule
    \end{tabular}%
    \label{tab:real-world-results}%
\end{table}%
